The Superposition of Diffusion Models Using the It\^o Density Estimator

The Cambrian explosion of easily accessible pre-trained diffusion models suggests a demand for methods that combine multiple different pre-trained diffusion models without incurring the significant computational burden of re-training a larger combined model. In this paper, we cast the problem of combining multiple pre-trained diffusion models at the generation stage under a novel proposed framework termed superposition. Theoretically, we derive superposition from rigorous first principles stemming from the celebrated continuity equation and design two novel algorithms tailor-made for combining diffusion models in SuperDiff. SuperDiff leverages a new scalable It\^o density estimator for the log likelihood of the diffusion SDE which incurs no additional overhead compared to the well-known Hutchinson's estimator needed for divergence calculations. We demonstrate that SuperDiff is scalable to large pre-trained diffusion models as superposition is performed solely through composition during inference, and also enjoys painless implementation as it combines different pre-trained vector fields through an automated re-weighting scheme. Notably, we show that SuperDiff is efficient during inference time, and mimics traditional composition operators such as the logical OR and the logical AND. We empirically demonstrate the utility of using SuperDiff for generating more diverse images on CIFAR-10, more faithful prompt conditioned image editing using Stable Diffusion, as well as improved conditional molecule generation and unconditional de novo structure design of proteins. https://github.com/necludov/super-diffusion

==> prompts/AND_diff_prompts.tex <==
\begin{tcolorbox}[breakable, colback=customwhite, colframe=customorange,title=Object and background prompts for diffusion models,    fontupper=\fontfamily{pcr}\selectfont\scriptsize]

\end{tcolorbox}

==> prompts/AND_vlm_prompt.tex <==
\cut{
\begin{tcolorbox}[breakable, colback=customwhite, colframe=customturq,title=GPT-4o prompt for evaluating compositional quality (from ~\citet{luo2024stylus}),    fontupper=\fontfamily{pcr}\selectfont\scriptsize]
\textbf{SYS PROMPT}
\\
You are a Photoshop expert judging which image has better composition quality.
\\ \\
Scoring: Compositional quality scores can be 2 (very high quality), 1 (visually aesthetic but has elements with distor- tion/missing features/extra features), 0 (low visual quality, issues with texture/blur/visual artifacts).
\\ \\
Composition can be broken down into three main aspects: \\
\begin{list}{}{\setlength{\leftmargin}{2em}}
 \item - Clarity: If the image is blurry, poorly lit, or has poor
composition (objects obstructing each other), it gets scores 0.
 \item - Disfigured Parts: This applies to both body parts of humans and animals as well as objects like motorcycles. If the image has a hand that has 6 fingers it gets a 1 for having otherwise normal fingers, but the hand should not have two fingers. If the fingers themselves are disfigured showing lips and teeth
warped in, it gets a 0. 
 \item - Detail: If the sail of a sailboat’s sail shows dynamic ripples
and ornate patterns, this shows detail and should get a score of 2. If it’s monochrome and flat, it gets a score of 1. If it looks like a cartoon and is inconsistent with the environment, give a score of 0.
\end{list}

\noindent\rule{\linewidth}{0.4pt} % This creates a horizontal line

\textbf{USER}
This is IMAGE A. Reply 'ACK'. \# Pass generated image from MODEL A

\noindent\rule{\linewidth}{0.4pt}

\textbf{USER}
This is IMAGE B. Reply 'ACK'. \# Pass generated image from MODEL B

\noindent\rule{\linewidth}{0.4pt}

\textbf{TASK PROMPT}
\\

Rate the quality of IMAGE A and IMAGE B. For each image, provide a score and explanation. \\

Image A Quality: <SCORE>(<EXPLANATION>) \\
Image B Quality: <SCORE>(<EXPLANATION>) \\
Preference: Image <CHOICE>(<EXPLANATION>)
\\ \\ 
I'll make my own judgement using your results, your response is just an opinion as part of a rigorous process. I provide additional requirements below:
\begin{list}{}{\setlength{\leftmargin}{2em}}
 \item  - You must pick an image for 'Better Quality', neither is not an option.
 \item - If it's a close call, make a choice first then explain why in parenthesis.
\end{list}
\end{tcolorbox}
}

==> scrap.tex <==
\begin{figure}[htbp]
    \centering
    % Define the spacing between columns
    \setlength{\spaceBetweenColumns}{0.2em} % Adjust as needed
    % Define the widths for label and image columns
    \setlength{\labelColumnWidth}{0.01\textwidth} % Adjust label column width
    \setlength{\imageColumnWidth}{0.9\textwidth}

    % Table with labels and images
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} >{\centering\arraybackslash}m{\imageColumnWidth}}

        % cat and dog
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"a cat"} and \textbf{"a dog"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/catdog(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/catdogs(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/sd_cat_dog.jpeg} \\

        % otter and duck
        \\
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"otter"} and \textbf{"duck"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/otterduck(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/otterduck(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/sd_otter_duck.jpeg} \\
    \end{tabular}

    \caption{Comparison of composition images generated by different methods for the given prompt inputs. For fair assessment, we use a combining prompt {\smaller \texttt{"that looks like"}} to link two concepts when prompting Stable Diffusion.}
    \label{fig:comparison1}
\end{figure}


\begin{figure}[htbp]
    \centering
    % Define the spacing between columns
    \setlength{\spaceBetweenColumns}{0.2em} % Adjust as needed
    % Define the widths for label and image columns
    \setlength{\labelColumnWidth}{0.01\textwidth} % Adjust label column width
    \setlength{\imageColumnWidth}{0.9\textwidth}

    % Table with labels and images
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} >{\centering\arraybackslash}m{\imageColumnWidth}}

        % avocado and chair
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"an avocado"} and \textbf{"a chair"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/avocadochair(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/avocadochair(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/sd_avovado_chair.jpeg} \\

        % pebbles and turtle
        \\
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"pebbles on a beach"} and \textbf{"a turtle"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/pebbleturtles(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/pebbleturtles(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/sd_pebbles_turtle.jpeg} \\
    \end{tabular}
    
    \caption{Comparison of composition images generated by different methods for the given prompt inputs.}
    \label{fig:comparison2}
\end{figure}


\begin{figure}[htbp]
    \centering
    % Define the spacing between columns
    \setlength{\spaceBetweenColumns}{0.2em} % Adjust as needed
    % Define the widths for label and image columns
    \setlength{\labelColumnWidth}{0.01\textwidth} % Adjust label column width
    \setlength{\imageColumnWidth}{0.9\textwidth}

    % Table with labels and images
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} >{\centering\arraybackslash}m{\imageColumnWidth}}

        % teddy bear and panda
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"teddy bear"} and \textbf{"panda"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/teddypanda(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/teddypanda(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/sd_teddy_panda.jpeg} \\

        % a donut and a map
        \\
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"a map"} and \textbf{"a donut"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/donutmap(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/donutmap(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/donutmap(SD).jpeg} \\
    \end{tabular}

    \caption{Comparison of composition images generated by different methods for the given prompt inputs.}
    \label{fig:comparison3}
\end{figure}


\begin{figure}[htbp]
    \centering
    % Define the spacing between columns
    \setlength{\spaceBetweenColumns}{2em} % Adjust as needed
    % Define the widths for label and image columns
    \setlength{\labelColumnWidth}{0.01\textwidth} % Adjust label column width
    \setlength{\imageColumnWidth}{0.9\textwidth}

    % Table with labels and images
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} >{\centering\arraybackslash}m{\imageColumnWidth}}

        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"a cat and a dog"}}
        \end{tcolorbox} \\[-0.5em]
        
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny } &
        \includegraphics[width=\linewidth]{figures/sd_base_and/and_sd_cat_dog.jpeg} \\[1em]

        % Second Row: Averaging Image
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"an otter and a duck"}}
        \end{tcolorbox} \\[-0.5em]
        
        \rotatebox{90}{\tiny } &
        \includegraphics[width=\linewidth]{figures/sd_base_and/and_sd_otter_duck.jpeg} \\[1em]

        % Third Row: Stable Diffusion Image
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"an avocado and a chair"}}
        \end{tcolorbox} \\[-0.5em]
        \rotatebox{90}{\tiny } &
        \includegraphics[width=\linewidth]{figures/sd_base_and/and_sd_avo_chair.jpeg} \\

    \end{tabular}

    \caption{Prompt editing using \texttt{\small `and'} as composing term.}
    \label{fig:prompt-edit-AND}
\end{figure}


\begin{figure}[htbp]
    \centering
    % Define the spacing between columns
    \setlength{\spaceBetweenColumns}{0.2em} % Adjust as needed
    % Define the widths for label and image columns
    \setlength{\labelColumnWidth}{0.01\textwidth} % Adjust label column width
    \setlength{\imageColumnWidth}{0.9\textwidth}

    % Table with labels and images
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} >{\centering\arraybackslash}m{\imageColumnWidth}}

        % dog and mountain
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"a mountain landscape"} and \textbf{"silhouette of a dog"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/dogmountain(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/dogmountain(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/sd_dog_mountain.jpeg} \\
    \end{tabular}
    
    \caption{Comparison of composition images generated by different methods for the given prompt inputs.}
    \label{fig:art1}
\end{figure}


\begin{figure}[htbp]
    \centering
    % Define the spacing between columns
    \setlength{\spaceBetweenColumns}{0.2em} % Adjust as needed
    % Define the widths for label and image columns
    \setlength{\labelColumnWidth}{0.01\textwidth} % Adjust label column width
    \setlength{\imageColumnWidth}{0.9\textwidth}

    % Table with labels and images
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} >{\centering\arraybackslash}m{\imageColumnWidth}}

        % dog and mountain
        & \begin{tcolorbox}[
            colback=custompurple,
            colframe=custompurple,
            coltext=white,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.5pt,
            left=2pt,
            right=2pt,
            top=2pt,
            bottom=2pt,
            width=0.9\textwidth,
            valign=center
        ]
            \centering
            {\small \textbf{"brazilian rainforest"} and \textbf{"a shape of a teapot"}}
        \end{tcolorbox} \\[-0.5em]
    
        % First Row: SuperDiff Image
        \rotatebox{90}{\tiny \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/foresttea(ours).jpeg} \\%[1em]

        % Second Row: Averaging Image
        \rotatebox{90}{\tiny \textbf{Averaging of Outputs}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/foresttea(avg).jpeg} \\%[1em]

        % Third Row: Stable Diffusion Image
        \rotatebox{90}{\tiny \textbf{Joint Prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_group_of_6_pics/foresttea(SD).jpeg} \\
    \end{tabular}
    
    \caption{Comparison of composition images generated by different methods for the given prompt inputs.}
    \label{fig:art2}
\end{figure}


\begin{figure}[htbp]
    \centering
    \newlength{\spaceBetweenColumns}
    \setlength{\spaceBetweenColumns}{0.3em} % Adjusted for visibility
    % Define the widths for label and image columns
    \newlength{\labelColumnWidth}
    \setlength{\labelColumnWidth}{0.01\textwidth}
    \newlength{\imageColumnWidth}
    \setlength{\imageColumnWidth}{(\textwidth - \labelColumnWidth - 6\spaceBetweenColumns) / 7}

    % Adjust column separation
    \setlength{\tabcolsep}{\spaceBetweenColumns}
    
    \begin{tabular}{>{\centering\arraybackslash}m{\labelColumnWidth} *{6}{>{\centering\arraybackslash}m{\imageColumnWidth}}}
        % First Row: Prompts
        & 
        {\scriptsize
        \begin{tcolorbox}[
            colback=customwhite,
            colframe=customwhite,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.05pt,
            left=1pt,
            right=1pt,
            top=1pt,
            bottom=1pt,
            width=\linewidth,
            height=0.8cm,
            valign=center
        ]
            \centering
            {\tiny `\textbf{a cat}' and `\textbf{a dog}'}
        \end{tcolorbox}
        } &
        {\scriptsize
        \begin{tcolorbox}[
            colback=customwhite,
            colframe=customwhite,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.05pt,
            left=1pt,
            right=1pt,
            top=1pt,
            bottom=1pt,
            width=\linewidth,
            height=0.8cm,
            valign=center
        ]
            \centering
            {\tiny `\textbf{otter}' and `\textbf{duck}'}
        \end{tcolorbox}
        } &
        {\scriptsize
        \begin{tcolorbox}[
            colback=customwhite,
            colframe=customwhite,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.05pt,
            left=1pt,
            right=1pt,
            top=1pt,
            bottom=1pt,
            width=\linewidth,
            height=0.8cm,
            valign=center
        ]
            \centering
            {\tiny `\textbf{an avocado}' and `\textbf{a chair}'}
        \end{tcolorbox}
        } &
        {\scriptsize
        \begin{tcolorbox}[
            colback=customwhite,
            colframe=customwhite,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.05pt,
            left=1pt,
            right=1pt,
            top=1pt,
            bottom=1pt,
            width=\linewidth,
            height=0.8cm,
            valign=center
        ]
            \centering
            {\tiny `\textbf{pebbles on a beach}' and `\textbf{a turtle}'}
        \end{tcolorbox}
        } &
        {\scriptsize
        \begin{tcolorbox}[
            colback=customwhite,
            colframe=customwhite,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.05pt,
            left=1pt,
            right=1pt,
            top=1pt,
            bottom=1pt,
            width=\linewidth,
            height=0.8cm,
            valign=center
        ]
            \centering
            {\tiny `\textbf{teddy bear}' and `\textbf{panda}'}
        \end{tcolorbox}
        } &
        {\scriptsize
        \begin{tcolorbox}[
            colback=customwhite,
            colframe=customwhite,
            fontupper=\fontfamily{pcr}\selectfont\scriptsize,
            arc=0.2em,
            boxsep=0.05pt,
            left=1pt,
            right=1pt,
            top=1pt,
            bottom=1pt,
            width=\linewidth,
            height=0.8cm,
            valign=center
        ]
            \centering
            {\tiny `\textbf{a donut}' and `\textbf{a map}'}
        \end{tcolorbox}
        } \\
        % Second Row: "Ours" Images
        \rotatebox{90}{\scriptsize \textbf{\textsc{SuperDiff}}} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_catdog(ours).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_otterduck(ours).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_avocadochair(ours).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_pebbleturtles(ours).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_teddypanda(ours).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_donutmap(ours).jpeg} \\
        
        % Third Row: "Baseline" Images
        \rotatebox{90}{\scriptsize \textbf{Average of scores}} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_catdogs(avg).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_otterduck(avg).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_avocadochair(avg).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_pebbleturtles(avg).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_teddypanda(avg).jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_donutmap(avg).jpeg} \\

        % Forth Row: "SD" Images
        \rotatebox{90}{\scriptsize \textbf{Joint prompting}} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_sd_cat_dog.jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_sd_otter_duck.jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_sd_avovado_chair.jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_sd_pebbles_turtle.jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_sd_teddy_panda.jpeg} &
        \includegraphics[width=\linewidth]{figures/sd_singles/single_donutmap(SD).jpeg} \\
    \end{tabular}
    \caption{Concept interpolations via different methods: \textsc{SuperDiff} (top row), the averaging of outputs with different prompts (middle row), and joint prompting with standard Stable Diffusion (SD) (bottom row) for six different prompt combinations. Here we use \name with the \texttt{AND} operation (sampling equal densities). 
    %For \name and averaging, we compose two conditional models that each condition on the individual concepts, i.e. \texttt{\smaller `a cat'} \texttt{\smaller `a dog'} respectively. To fairly compare with SD, we augment the prompts such that they best mimic the compositional operation of the \textsc{SuperDiff} and averaging methods. We use a combining prompt {\smaller \texttt{`that looks like'}} to link two concepts --- for the example in the first column, we prompt SD with {\smaller \texttt{`a cat that looks like a dog'}}.
    }
    \label{fig:comparison}
\end{figure}

==> tables/protein_AND_logp_ablation.tex <==
\begin{table}[h!]
%\vspace{-15pt}
    \centering
    \caption{Ablation of the bias ($\ell$) parameter for combining Proteus and FrameDiff scores using \name(\AND).}
    %\vspace{-1em}  
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrrrrrr}
            \toprule
            &  \multicolumn{2}{c}{\textbf{Designability}} & \multicolumn{3}{c}{\textbf{Novelty}} & \multicolumn{3}{c}{\textbf{Diversity}} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
            %\midrule
             $\ell$ &
            \makecell{$< 2\text{\r{A} \texttt{scRMSD}}$ \\$ (\uparrow)$} & \makecell{Avg. \texttt{scRMSD} \\ $(\downarrow)$} & \makecell{$< 0.5$ \texttt{scTM} \\  $(\uparrow)$ } & \makecell{$< 0.3$ \texttt{scTM} \\  $(\uparrow)$} & \makecell{Max. \texttt{scTM} \\$(\downarrow)$} & \makecell{Frac. $\beta$ \\ $(\uparrow)$} & \makecell{Pairwise \texttt{scTM} \\$(\downarrow)$} & \makecell{Max. cluster \\$(\uparrow)$}\\
            \midrule
             $0$ & $0.740 \pm 0.03$ & $2.119 \pm 0.16$ & $0.320 \pm 0.03$ & $0.044 \pm 0.01$ & $0.513 \pm 0.01$ & $0.142 \pm 0.01$ & $0.310 \pm 0.02$ & $0.265 \pm 0.01$ \\
            $1$ & $0.776 \pm 0.03$ & $1.986 \pm 0.15$ & $0.336 \pm 0.03$ & $0.020 \pm 0.01$ & $0.521 \pm 0.01$ & $0.137 \pm 0.01$ & $0.308 \pm 0.01$ & $0.242 \pm 0.01$ \\
            $10$& $0.808 \pm 0.03$ & $1.747 \pm 0.14$ & $0.348 \pm 0.03$ & $0.020 \pm 0.01$ & $0.521 \pm 0.01$ & $0.119 \pm 0.01$ & $0.310 \pm 0.01$ & $0.269 \pm 0.02$ \\
            $20$ & $0.876 \pm 0.02$ & $1.402 \pm 0.12$ & $0.388 \pm 0.03$ & $0.040 \pm 0.01$ & $0.512 \pm 0.01$ & $0.101 \pm 0.01$ & $0.313 \pm 0.01$ & $0.220 \pm 0.02$ \\ 
            $30$ & $0.912 \pm 0.02$ & $1.294 \pm 0.16$ & $0.356 \pm 0.03$ & $0.044 \pm 0.01$ & $0.530 \pm 0.01$ & $0.093 \pm 0.01$ & $0.316 \pm 0.01$ & $0.211 \pm 0.02$ \\
            $40$ & $0.928 \pm 0.02$ & $1.169 \pm 0.10$ & $0.312 \pm 0.03$ & $0.024 \pm 0.01$ & $0.548 \pm 0.01$ & $0.081 \pm 0.01$ & $0.328 \pm 0.01$ & $0.207 \pm 0.02$\\
            $50$ & $0.948 \pm 0.01$ & $1.058 \pm 0.07$ & $0.324 \pm 0.03$ & $0.008 \pm 0.01$ & $0.566 \pm 0.01$ & $0.075 \pm 0.01$ & $0.340 \pm 0.01$ & $0.211 \pm 0.03$ \\
            $60$ & $0.904 \pm 0.02$ & $1.192 \pm 0.08$ & $0.308 \pm 0.03$ & $0.040 \pm 0.01$ & $0.568 \pm 0.01$ & $0.072 \pm 0.01$ & $0.357 \pm 0.02$ & $0.192 \pm 0.02$ \\
            $100$ & $0.868 \pm 0.02$ & $1.506 \pm 0.16$ & $0.296 \pm 0.03$ & $0.020 \pm 0.01$ & $0.572 \pm 0.01$ & $0.060 \pm 0.01$ & $0.397 \pm 0.05$ & $0.161 \pm 0.03$\\
            $200$ & $0.644 \pm 0.03$ & $2.909 \pm 0.24$ & $0.288 \pm 0.03$ & $0.024 \pm 0.01$ & $0.545 \pm 0.01$ & $0.048 \pm 0.01$ & $0.295 \pm 0.09$ & $0.197 \pm 0.04$ \\
            \bottomrule
        \end{tabular} 
        }
        \label{table:prot_AND_abl}
\end{table}

==> tables/protein_OR_temp_logp_ablation.tex <==
\begin{table}[h!]
%\vspace{-15pt}
    \centering
    \caption{Ablation of temperature ($T$) and bias ($\ell$) parameters for combining Proteus and FrameDiff scores using \name(\OR).}
    %\vspace{-1em}  
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{llrrrrrrrr}
            \toprule
            & & \multicolumn{2}{c}{\textbf{Designability}} & \multicolumn{3}{c}{\textbf{Novelty}} & \multicolumn{3}{c}{\textbf{Diversity}} \\
            \cmidrule(lr){3-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
            %\midrule
            $T$ & $\ell$ &
            \makecell{$< 2\text{\r{A} \texttt{scRMSD}}$ \\$ (\uparrow)$} & \makecell{Avg. \texttt{scRMSD} \\ $(\downarrow)$} & \makecell{$< 0.5$ \texttt{scTM} \\  $(\uparrow)$ } & \makecell{$< 0.3$ \texttt{scTM} \\  $(\uparrow)$} & \makecell{Max. \texttt{scTM} \\$(\downarrow)$} & \makecell{Frac. $\beta$ \\ $(\uparrow)$} & \makecell{Pairwise \texttt{scTM} \\$(\downarrow)$} & \makecell{Max. cluster \\$(\uparrow)$}\\
            \midrule
            \multirow{4}{*}{$1$} & $0$ & $0.752 \pm 0.03$ & $1.940 \pm 0.14$ & $0.276 \pm 0.03$ & $0.008 \pm 0.01$ & $0.547 \pm 0.01$ & $0.147 \pm 0.01$ & $0.309 \pm 0.02$ & $0.268 \pm 0.02$ \\
            & $1e-1$ & $0.820 \pm 0.02$ & $1.620 \pm 0.11$ & $0.316 \pm 0.03$ & $0.020 \pm 0.01$ & $0.532 \pm 0.01$ & $0.139 \pm 0.01$ & $0.307 \pm 0.01$ & $0.259 \pm 0.02$ \\
            & $1$& $0.976 \pm 0.01$ & $0.929 \pm 0.05$ & $0.396 \pm 0.03$ & $0.024 \pm 0.01$ & $0.528 \pm 0.01$ & $0.127 \pm 0.01$ & $0.307 \pm 0.02$ & $0.246 \pm 0.03$  \\
            \midrule
            \multirow{4}{*}{$10$} & $0$ & $0.700 \pm 0.03$ & $2.309 \pm 0.18$ & $0.276 \pm 0.03$ & $0.028 \pm 0.01$ & $0.534 \pm 0.01$ & $0.147 \pm 0.01$ & $0.299 \pm 0.01$ & $0.299 \pm 0.02$\\
            & $1e-1$ & $0.904 \pm 0.02$ & $1.137 \pm 0.07$ & $0.384 \pm 0.03$ & $0.032 \pm 0.01$ & $0.530 \pm 0.01$ & $0.120 \pm 0.01$ & $0.308 \pm 0.01$ & $0.240 \pm 0.02$  \\
            & $1$& $0.948 \pm 0.01$ & $0.976 \pm 0.06$ & $0.400 \pm 0.03$ & $0.028 \pm 0.01$ & $0.532 \pm 0.01$ & $0.119 \pm 0.01$ & $0.311 \pm 0.01$ & $0.221 \pm 0.02$ \\
            \midrule
            \bottomrule
        \end{tabular} 
        }
        \label{table:prot_OR_abl}
\end{table}

==> tables/protein_avg_kappa_ablation.tex <==
\begin{table}[t]
%\vspace{-15pt}
    \centering
    \caption{stuff}
    %\vspace{-1em}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrrrrrrr}
            \toprule
             & \multicolumn{2}{c}{\textbf{Designability}} & \multicolumn{3}{c}{\textbf{Novelty}} & \multicolumn{3}{c}{\textbf{Diversity}} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
            %\midrule
             $\kappa$ &
            \makecell{$< 2\text{\r{A} \texttt{scRMSD}}$ \\$ (\uparrow)$} & \makecell{Avg. \texttt{scRMSD} \\ $(\downarrow)$} & \makecell{$< 0.5$ \texttt{scTM} \\  $(\uparrow)$ } & \makecell{$< 0.3$ \texttt{scTM} \\  $(\uparrow)$} & \makecell{Max. \texttt{scTM} \\$(\downarrow)$} & \makecell{Frac. $\beta$ \\ $(\uparrow)$} & \makecell{Pairwise \texttt{scTM} \\$(\downarrow)$} & \makecell{Max. cluster \\$(\uparrow)$}\\
             \midrule
             $0.1$ & $0.488 \pm 0.03$ & $3.520 \pm 0.21$ & $0.188 \pm 0.03$ & $0.020 \pm 0.01$ & $0.555 \pm 0.01$ & $0.172 \pm 0.01$ & $0.310 \pm 0.01$ & $0.278 \pm 0.01$ \\
             $0.2$ & $0.568 \pm 0.03$ & $3.148 \pm 0.21$ & $0.216 \pm 0.03$ & $0.036 \pm 0.01$ & $0.530 \pm 0.01$ & $0.165 \pm 0.01$ & $0.321 \pm 0.02$ & $0.287 \pm 0.02$\\
             $0.3$ & $0.596 \pm 0.03$ & $2.690 \pm 0.18$ & $0.228 \pm 0.03$ & $0.016 \pm 0.01$ & $0.545 \pm 0.01$ & $0.162 \pm 0.01$ & $0.318 \pm 0.02$ & $0.263 \pm 0.01$\\
             $0.4$ & $0.676 \pm 0.03$ & $2.837 \pm 0.20$ & $0.288 \pm 0.03$ & $0.028 \pm 0.01$ & $0.524 \pm 0.01$ & $0.152 \pm 0.01$ & $0.321 \pm 0.02$ & $0.274 \pm 0.02$ \\
             $0.5$ & $0.740 \pm 0.03$ & $1.960 \pm 0.14$ & $0.360 \pm 0.03$ & $0.024 \pm 0.01$ & $0.511 \pm 0.01$ & $0.139 \pm 0.01$ & $0.310 \pm 0.01$ & $0.253 \pm 0.01$\\
             $0.6$ & $0.896 \pm 0.02$ & $1.258 \pm 0.08$ & $0.412 \pm 0.03$ & $0.048 \pm 0.01$ & $0.515 \pm 0.01$ & $0.139 \pm 0.01$ & $0.304 \pm 0.01$ & $0.254 \pm 0.01$\\
             $0.7$ & $0.908 \pm 0.02$ & $1.174 \pm 0.07$ & $0.404 \pm 0.03$ & $0.028 \pm 0.01$ & $0.523 \pm 0.01$ & $0.132 \pm 0.01$ & $0.306 \pm 0.01$ & $0.254 \pm 0.02$ \\
             $0.8$ & $0.948 \pm 0.01$ & $1.007 \pm 0.05$ & $0.388 \pm 0.03$ & $0.052 \pm 0.01$ & $0.526 \pm 0.01$ & $0.128 \pm 0.01$ & $0.307 \pm 0.02$ & $0.229 \pm 0.02$\\
             $0.9$ & $0.952 \pm 0.01$ & $0.994 \pm 0.06$ & $0.416 \pm 0.03$ & $0.028 \pm 0.01$ & $0.527 \pm 0.01$ & $0.124 \pm 0.01$ & $0.306 \pm 0.01$ & $0.244 \pm 0.02$ \\
            \bottomrule
            
        \end{tabular}
    }
    %\vspace{-15pt}
    \label{table:prot_avg_kappa_abl}
\end{table}

